Exploring Highly Quantised Neural Networks for Intrusion Detection in Automotive CAN

Vehicles today comprise intelligent systems like connected autonomous driving and advanced driving assistance systems (ADAS) to enhance the driving experience, which is enabled through increased connectivity to infrastructure and fusion of information from different sensing modes. However, the rising connectivity coupled with the legacy network architecture within vehicles can be exploited for launching active and passive attacks on critical vehicle systems and directly affecting the safety of passengers. Machine learning-based intrusion detection models have been shown to successfully detect multiple targeted attack vectors in recent literature, whose deployments are enabled through quantised neural networks targeting low-power platforms. Multiple models are often required to simultaneously detect multiple attack vectors, increasing the area, (resource) cost, and energy consumption. In this paper, we present a case for utilising custom-quantised MLP's (CQMLP) as a multi-class classification model, capable of detecting multiple attacks from the benign flow of controller area network (CAN) messages. The specific quantisation and neural architecture are determined through a joint design space exploration, resulting in our choice of the 2-bit precision and the n-layer MLP. Our 2-bit version is trained using Brevitas and optimised as a dataflow hardware model through the FINN toolflow from AMD/Xilinx, targeting an XCZU7EV device. We show that the 2-bit CQMLP model, when integrated as the IDS, can detect malicious attack messages (DoS, fuzzing, and spoofing attack) with a very high accuracy of 99.9%, on par with the state-of-the-art methods in the literature. Furthermore, the dataflow model can perform line rate detection at a latency of 0.11 ms from message reception while consuming 0.23 mJ/inference, making it ideally suited for integration with an ECU in critical CAN networks.

==> archBackup.tex <==
\section{Algorithm and Architecture}\label{sec:architecture}
A tree-based reduction logic can fully exploit the inherent data-parallelism available in the reduction operation. It is the fastest way to reduce vector/vectors of scalar data points to a single value. The tree-based method restricts that the vector size has to be a power of 2. Generalizing it to any arbitrary size is a challenge. We propose a generalized tree reduction method which we realize in the FPGA hardware. 

\subsection{Algorithm}
Generalizing a tree reduction is done in two phases: a distribution phase and a merging phase. We reduce more than one vector in parallel. In the distribution phase, the vectors are split into partitions. Equal sized partitions from different vectors are grouped, laid over a reduction tree, and reduced in parallel. The reduced value from different partitions belonging to the same vector is merged either using tree nodes or a shift-and-add sequence of operations. 




Our algorithm is divided into three phases: configure phase, distribution phase and merging phase. In configure phase, configuration values are streamed on the FPGA from host. In distribution phase, a binary tree is employed, called a routing tree network. This tree is used to distribute multiple input vectors of equal but arbitrary length to route input data (encapsulating all the values of vectors) on the base level (leaf level) in a particular fashion. Finally, in merging phase, an inverted binary tree, called a merging tree network, is utilized with some additional route and accumulate logic to reduce the vectors according to target application. \par

Each node of routing tree network has a vector present on its incoming and two outgoing edges. All the nodes store two left-shift values, which are used on the incoming edge vector, to independently generate vectors for each outgoing edge. This vector distribution method leads to a particular distribution of vector-values at the base level, where each leaf carries a scalar value. 
% This particular vector distribution method applied on input vectors enable reduction through merging tree network.  

\subsubsection{Vector Distribution Method}
Vector Distribution Method is a partition-based distribution method, where vector is partitioned and then distributed at partition level. 
% First, we look at the underlying method, employed for a single vector's partition and distribution by the routing tree network and then at the distribution with multiple vectors. 
Consider we have $n$ vectors each of size $m$, each vector is denoted by $v\textsubscript{i}$ where $i = 1,2,\cdots,n$. 
We know mathematically, every number can be expressed as a sum of different powers of two. For example: 15 can be partitioned into $8\; (2^{3}),\; 4\; (2^{2}),\; 2\;(2^{1}), \;and\; 1\;(2^{0})$. Similarly, each vector is partitioned into $j$ partitions and the size of each partition being a different power of two. We denote each partition as $p\textsubscript{i}$ where $i = 1,2,\cdots,j$. 
The partitions of the vector $v\textsubscript{i}$ follows the following condition: $|p\textsubscript{i1}| > |p\textsubscript{i2}| > \cdots > |p\textsubscript{ij}|$ (here $|.|$ represents the size of the partition). 
% Moreover, atleast $n \times m$ leaves are required at the base level.  Similarly, vector of size $m$ is divided into $j$ partitions with each partition's size being a different power of two.
At the base of routing tree network, vector is organised (moving from left to right) by sorting the vector-partitions in decreasing order of size. \par
%% do I need to write in math mode

In case of multiple vectors, each vector follows the same partition method discussed in last paragraph. However, distribution at the base level of routing tree network changes with multiple vectors. For multiple vectors, partitions of same size across vectors are grouped together and then the groups are sorted in decreasing order of partition size. All applications follow this group-wise distribution method, but within the group, distribution varies with application. 


\begin{figure}
\centering
\includegraphics[scale=0.9]{figures/microExample.eps}
\caption{The figure shows the same PE structure used for a single run configurations. In part (a), two 2x2 convolutions are executed in parallel. In part (b), two 1x3 convolutions are performed over the same structure. The shift amounts are written as tuples over the routing tree nodes.}
\label{fig:sum_example}
\end{figure}

For calculating the sum of elements of a vector, within a group, partitions of $n$ vectors are placed sequentially in a particular order and this order is maintained within the other groups. In Figure \ref{fig:sum_example}, we have 2 vectors \textbf{X} and \textbf{V} each of size 7. We call their partitions of size 4, 2, and 1 as $p\textsubscript{11}$, $p\textsubscript{12}$, $p\textsubscript{13}$ for \textbf{X} and $p\textsubscript{21}$, $p\textsubscript{22}$, $p\textsubscript{23}$ for \textbf{V}. The routing tree network organises these vectors' partitions at the base level in the following manner $p\textsubscript{11}$, $p\textsubscript{21}$, $p\textsubscript{12}$, $p\textsubscript{22}$, $p\textsubscript{13}$, $p\textsubscript{23}$, meaning partitions of size 4 appear first followed by group of partition size, 2 and 1. For dot product, within a group, elements of partitions' between whom dot product has to be performed are placed alternatively and the same order is followed within the other groups as well. In Figure \ref{fig:dot_example}, we have 2 vectors \textbf{X} and \textbf{V} of size 4 and each vector has a partition of size 4. In the level lying above MUL level, we can see both 4-size partition are grouped together and elements of partitions are placed alternatively to perform multiplication followed by addition in below layers to complete dot product.
% (but alternately values needs to be distributed dot product refer fig2b and 3)
% \subsubsection{Rationale behind partition strategy}
% The strategy to partition a vector into powers of two, encapsulates the fundamental behaviour of binary tree which is merging of two nodes, therefore facilitates vector reduction.  

\subsubsection{Vector Merging Method}
In the merging tree network, partitions belonging to same vectors are merged to generate $n$ reduced values parallely. We know binary tree reductions work smoothly for even sized vectors. 
% The first $n$ nodes of the last level of merge tree contains non-interfered correct values. 
The proposed partition-based distribution strategy exploits this property by creating partition of sizes of power of 2. 
% Even with an odd size vector which will have an odd size partition, when two is raised by power 0.   
% binary tree reduction's property 
% of merging two (even number) nodes to create a single odd node. 
% Each tree node receives input over two edges, and performs reduction operation on the values. 
% Therefore, initially at first level, merging tree reduces even size partitions of distinct vectors. 
For even size partition, no interference occurs between two nodes belonging to different vectors. For odd size partition ($2^0$), however, interference occurs between nodes of different vectors. The problem of interference begins from the first level itself if a partition of size 1 exists. Although it may seem like the problem will not appear if we do not have a partition of size 1 but that is not true. Whenever the partition size is reduced to size 1 down the tree, partition becomes a candidate for interference. For instance, partitions of size $2,\,4,\,8,\,16, \cdots$ are reduced to partitions of size 1 in $1^{st},\,2^{nd},\,3^{rd},\,4^{th},\cdots$ levels, respectively. Our algorithm solves this interference problem, arising due to odd size partition, by introducing a tree tapping\footnote{Tree Tapping is used analogous to phone tapping, here it means value is read and transmitted.} technique. This tree tapping technique works by utilizing the route and accumulate logic. All the single element partitions of a level are tapped and left-shifted\eqref{shift_val} such that they align with the nodes of their corresponding vectors for addition. 

% Additionally, left-shifted levels are passed through a mask before addition to convert all nodes to zero except the nodes corresponding to partitions of size 1. A separate route and accumulate logic is employed for shifting, masking, and addition of shifted-masked level and next level. Eventually, single element partitions are converted into garbage in next levels, but ultimately, first $n$ nodes contain correct but incomplete values at the $log(|P_{i1}|)$ level. This level is added with last level's shifted-masked values in route and accumulate logic to produce final output.\par

Following a particular distribution strategy not only gives a consistent distribution, but also enables us to design hardware of the merging tree network with predictable \textit{shift values (SV)}. The shift value is calculated with the below formula, where $l$ represents levels of reduction tree, indexed with top level as 0 and increments as we move down the tree. 

\begin{equation}\label{shift_val}SV\left( {l} \right) = ({{n}} \times 2^{(log(|P_{i1}|)-l)}) \end{equation}


\subsection{Architecture}
We propose a hardware architecture made-up of two binary tree networks where the top tree executes distribution phase and the bottom tree executes the merging phase as shown in Figure \ref{fig:sum_example}. Both the trees connect at the base of the tree (leaf level). We define total leaves present at the base level as \textit{Local Compute Size (LCS)}, hence the depth/height of each tree is $log_2 (LCS)$. \par


\subsubsection{Routing Tree Network}

% The main aim of the routing tree network is to perform partition-based distribution to provide a required distribution at base level. In configure phase, each edge is configured by the host with a left-shift value. Each node receives a vector on its input edge and forwards it on the output edges by left shifting the input vector with corresponding values. To support all types of distribution, a shift register equal to the input data length is present on both edges of each node except the base level nodes. Through these shifts, on a root to leaf path, a particular vector value is routed to one of the leaves. For example, the value $v_0$ is routed to the fifth leaf in Figure~\ref{fig:sum_example} by left shifting the original vector $v_0,\cdots,v_6$, 4 times over 3 routing nodes. 

The main aim of the routing tree network is to perform partition-based distribution to provide a required distribution at base level. In configure phase, each edge is configured by the host with a left-shift value. Each node has a vector of input data length and while traversing the tree, vectors are left shifted by values present on the edges. To support all types of distribution, a register equal to the input data length is present on all nodes except the base level nodes. Through these shifts, a particular vector value is routed from the root to one of the leaves. For example, the value $v_0$ is routed to the fifth leaf in Figure~\ref{fig:sum_example} by left shifting the original vector $v_0,\cdots,v_6$, 4 times over 3 routing nodes. 
% Observe that feature maps vectors can be replicated across nodes using a shift value of 0 on both the output edges.
Using a tree network reduces the fan-out in our architecture. More precisely, for a input vector of size $m$, the fan-out reduces from $m \times LCS$ to  $2m$ between a flat and hierarchical tree-based routing.

% The host configures each routing node with shift amounts. Figure~\ref{fig:pexample} shows two-run configurations of the same architecture with different vector sizes. In part (a), since the vector of size 4 is already a power of 2, it does not need partitioning and is mapped on the leaves for reduction by merging tree network. In part (b), the feature vector $x_0, x_1, x_2$, is split into 2 partitions, $x_0,x_1$ and $x_2$ and similarly $v_0, v_1, v_2$ is partitioned. 




\subsubsection{Merging Tree Network}

The merging tree network comprises of two synchronous pipelines running in parallel. We call these two pipelines: \textit{Reduction Tree (RT)} and \textit{Route And Accumulate (RA)}. \textit{RT} pipeline implements a binary tree where each level of binary tree is realized as a pipeline stage. Each pipeline stage comprises of reduction operator between every two nodes. Values present on the input edges are stored in registers and its utilization reduces by half every stage, as we descend the tree.\par

\textit{RA} pipeline has same number of stages as the \textit{RT} pipeline where each stage has a shift, mask, and add operation unit. The pipeline taps every stage of \textit{RT} pipeline to read one-sized partitions. 
% As we have seen, tapping is necessary, because otherwise, if we wait to read them in subsequent levels, they will merge with other vector's partition of size 1 to generate distorted values. 
The tapping mechanism is carried-out by making a copy of data present in \textit{RT} pipeline in another register present in \textit{RA} pipeline. For instance, when first level's data is copied, in the same clock cycle, copied vector is shifted\eqref{shift_val} and a mask is applied(How?). In the next clock cycle, second level of reduction tree is tapped and is ready for addition with previous level's shifted-masked vector. During this same clock cycle, after addition, resultant vector is shifted\eqref{shift_val} and masked as well, to make it available in next clock cycle for addition with third level's tapped data and so on. 






% \begin{figure*}
% \centering
% \includegraphics[scale=1]{figures/example.eps}
% \caption{The figure shows the same PE structure used in two-run configurations. In part (a), two 2x2 convolutions are executed in parallel. In part (b), two 1x3 convolutions are performed over the same structure. The shift amounts are written as tuples over the routing tree nodes.}
% \label{fig:pexample}
% \end{figure*}
\begin{figure}
\centering
\includegraphics[scale=1]{figures/dotPro.eps}
\caption{Block diagram of the Processing Engine in our accelerator. The PE is made of two trees connected at the base through an array of DSP multipliers. The PE is fully pipelined to produce output every cycle.}
\label{fig:dot_example}
\end{figure}



==> architecture-fpl.tex <==
\section{System Architecture}\label{sec:architecture-fpl}
\subsection{Hybrid-FPGA based IDS capable ECU}
% Figure~\ref{fig:arch} shows the overview of the proposed hybird FPGA based ECU architecture on a Xilinx Zynq Ultrascale+ device. 
% Incoming CAN packet bits are decoded by the CAN Controller on the Programmable System (PS). 
% The ID of each message is then extracted and sent to the Programmable Logic region (PL) via the Advanced eXtensible Interface (AXI) interconnect. 
% Here, the IDS processes and classifies them into either normal or an attack message. 

Figure~\ref{fig:arch} shows an overview of the proposed hybrid-FPGA based distributed ECU architecture on a Xilinx Zynq Ultrascale+ device.
The Zynq Ultrascale+ device integrates a quad-core ARM processor and a dual-core ARM real-time core within the processing system (PS) section of the device, along with integrated peripherals and interfaces.
The programmable logic (PL) section of the device enables the addition of specialised custom logic blocks or accelerators that can be accessed using the Advanced eXtensible Interface (AXI) protocol from the PS.
In this architecture, standard ECU function(s) are mapped as software tasks onto the ARM cores on the PS, on top of a standard operating system like petalinux or a real-time operating system. 
The operating system provides relevant drivers and APIs for accessing the PS peripherals and the PL accelerators, abstracting away low-level details of these blocks to create an AUTOSAR compliant architecture~\cite{fons2012fpga}.

In our approach, we propose to use the integrated CAN interface on the PS to handle the interfacing of ECU to the CAN bus, as shown in Figure~\ref{fig:arch}.
%CAN network packets  handled by the integrated CAN controller on the PS that attaches the ECU to the CAN bus.
%As shown in Figure~\ref{fig:arch}, CAN network packets are handled by the integrated CAN controller on the PS that attaches the ECU to the CAN bus.
Any received packets at the interface are read by the software tasks on the PS and further processed based on the ECU's task specification.
In tandem, the IDS task extracts relevant packet feature information from the received packet and forwards it to the IDS accelerator through the integrated APIs.
For this evaluation, we have used the off-the-shelf DPU accelerator as the IDS inference engine, which executes our TensorFlow ML model. % shown in Figure~\ref{fig:2}. 
Standard Vitis AI Runtime (VART) APIs are used to configure and communicate with the IDS engine.
The model uses interrupts to indicate the completion of tasks to the PS, allowing the software tasks to run in a non-blocking fashion.
This approach allows for seamless integration of the IDS API calls with the other event/time-triggered tasks to be executed by the ECU.
For high-performance networks like Automotive Ethernet, the IDS model can be configured to directly read the packets from the interface (also in PL), eliminating the bottleneck caused by the software-based data movement. 
In this case, the IDS task would enable the accelerator operation at the startup phase of the network and would be interrupted only when an anomaly is observed in the network traffic. 

\begin{figure}[t!]
    \centering
    \includegraphics[scale = 0.65]{figures/FPL-23-SD.pdf}
    \caption{Proposed system architecture of the IDS-ECU. The ML model is accelerated on the PL part of the FPGA device.}
    \label{fig:arch}
    \vspace{-10pt}
\end{figure}

\subsection{Dataset \& Training}
We use the CAR Hacking dataset for training and testing our model~\cite{song2020vehicle}.
The dataset provides a labelled set of normal and attack messages which were captured via the Onboard Diagnostic (OBD) port in an actual vehicle, with attack messages injected in real-time. 
The dataset includes generalised DoS and Fuzzing message injections (as well as other targeted attacks gear-ECU spoofing) allowing us to validate the detection accuracy across these different attacks. 
DoS attacks flood the bus with a higher priority message when injected while a fuzzing attack transmits messages with random IDs and payloads at random intervals to disrupt the normal flow of messages. 
%DoS attack involves flooding the bus with high-priority '0x000' ID messages. 
%Fuzzing involves sending random messgaes with random ID's and payloads.
%Being a more general attack, it pushes the model to accurately learn the normal messages to detect intrusions. 
%We chose not to model the spoofing attacks as they are very specific and not generalisable as the attacks target a specific ECU with a fixed payload contents. 
An extract from the dataset is shown in table~\ref{table:4}, showing the CAN ID (ID field), control field, and the actual data segment.
We ignored targeted attacks in the dataset since they are modelled by a constant message sequence (specific ID and payload) and is not generalisable to other ECUs.

As our input feature, we use a window approach to capture adjacent sequences of CAN messages, which are fed as input to the machine learning model to capture the correlation between messages under different operating conditions.
Through design space exploration, we observed that a window of 4 successive CAN-IDs provided optimal performance and was hence chosen for our implementation. 
For training, we pre-process the dataset to feed this windowed sequence as the model's input, while in the implementation, this was mapped as a FIFO style buffer stacking sequential CAN IDs to form the input tensor for the IDS.  
%We pre-process the dataset prior to training to mimic the dataflow the model will obtain as its input, when integrated into the ECU. 
%To achieve this, each message is converted to the equivalent binary value (modeling reception from the CAN interface) from which the ID's are extracted. 
%To generate our FIFO-style operation, groups of \textit{n} sequential IDs are stacked to form the input tensor for the IDS. 
%We set the value of \textit{n} as 4 for both DoS and Fuzzing attacks for optimal performance based on our observation from the design space exploration step.
%Each layer of this stack forms the combined input shape for the first layer, which is reshaped to feed into the exact channels for training and testing.

To train the model, we used the adam optimizer with the binary cross-entropy loss function.
The learning rate was set at 0.0001 during the entire training process to reduce any performance degradation when quantising the network post-training as observed in~\cite{wu2018training}.
%A small learning rate helps in the reducing performance degradation when quantising a pre-trained network~\cite{wu2018training}.
We first train the model on DoS attack and ensure optimal performance; subsequently, this trained model is trained on the fuzzing dataset to improve generalisation across the two attack modes through inductive transfer. 
%This model is then used as a starting point and trained on the Fuzzing dataset. 
This model file is then tested in both the DoS \& Fuzzing attacks to ensure there was no performance degradation.
The model saves intermediate results at each epoch allowing us to progressively track and integrate early stopping in case of a significant drop in the accuracy.
The model was trained for 25 epochs with a batch size of 64 and the dataset was split as 80:15:5 for training, validation and testing respectively for both attacks to allow a sufficient amount of information for training and fine-tuning the quantised network. 
%
%In both cases, model instances with higher validation accuracy during training were progressively saved and the one with the highest performance was used for testing. \todo[inline]{I do not %understand this line... }
%The model was trained for 25 epochs with a batch size of 64.
%Early stopping mechanisms in place that were based on the validation loss metric.
%We split the dataset as 80:15:5 for training, validation, and testing respectively, allocating the large section to training for optimisation of the quantised network.

\begin{table}[t!]
\centering
\caption{An extract from the open Car hacking dataset which is used for our testing and evaluation.}
\scalebox{0.95}{
\begin{tabular}{@{}lrrr@{}}
\toprule
\textbf{Time}     & \textbf{ID} & \textbf{DLC} & \textbf{Data}           \\ \midrule
\textbf{$\ldots$} \\
1478198376.389427 & 0316            & 8            & 05,21,68,09,21,21,00,6f \\
1478198376.389636 & 018f            & 8            & fe,5b,00,00,00,3c,00,00 \\
1478198376.389864 & 0260            & 8            & 19,21,22,30,08,8e,6d,3a \\ 
\textbf{$\ldots$} \\
\bottomrule
\end{tabular}}
\label{table:4}
\end{table}

\subsection{Proposed Model}
\todo[inline]{Dropout for now looks like does not help the training of a qunatised model. Lets see if that is. Also explore what is the impact of batchnormalization on model training.}
To determine the model configuration with minimal computational complexity, we explored different network architectures that combine the layers supported by the Vitis-AI flow. 
Each model was defined in TensorFlow (TF) using standard TF functions and nodes. % \todo[inline]{Which attack did we use? Also, did we use the latency as a measure?}
We evaluated different models comparing their inference latency and detection accuracy across both attack datasets when mapped using the Vitis-AI to determine our lightweight network model to implement. 
%
%We use the sequence of \textit{n} successive IDs from the attack datasets as the input from which the model learns optimal features.
%Based on the design space exploration and the layers supported by the Vitis-AI framework,  we choose CNN which provides the best combination of accuracy and computational efficiency.
Our chosen model is composed of 5 \textit{Conv2D} layers implemented with 40, 80, 120, 160 \& 200 filters at each layer, each filter having a dimension of 3x3. 
This is followed by a \textit{Flatten} and 2 \textit{Dense} layers implemented with \{32, 1\} units respectively. 
The final dense layer consists of \textit{sigmoid} activation to predict the probability of an attack message.
In addition, batch normalisation and dropout layers were used between the convolutional layers to prevent overfitting and to improve learning efficiency during the inductive training phase.

==> experiments-fpl.tex <==
\section{Deployment and Experimental Results}\label{exp_results-fpl}
\todo[inline]{Include the training and validation loss plots as grpahs here.}
%We use the testing split of our dataset to report our model performance numbers.
Once the model was chosen, it was trained using an Nvidia RTX A6000 GPU using the training split of the dataset(s), starting with the DoS attacks and subsequently moving to the fuzzing attacks. 
The pre-quantisation accuracy is then verified using the test split of the dataset and is shown in Table~\ref{table:preqcomp}.
%It is then trained on a GPU until and it's performance verified for attack detection as shown in Table~\ref{table:preqcomp}.
The exported model file is passed to the Vitis-AI tool flow which quantise the model, weights, biases, and activations to 8-bit precision, followed by an optional post-quantisation fine-tuning step to account for any performance degradation from the quantisation. 
In our case, the post-quantisation fine-tuned model performance showed no visible degradation in inference performance as shown in Table~\ref{table:preqcomp}. 
\begin{table}[t!]
\centering
\caption{Inference accuracy metrics of the proposed MA-QCNN model, pre and post quantisation on the two attacks.} %\todo{we could replace post-Q as QdCNN?}
\scalebox{0.95}{%0.85
\begin{tabular}{@{}lllllll@{}}
\toprule
\textbf{Attack} & \textbf{Model}  & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{FPR} & \textbf{FNR} \\
\midrule
\multirow{2}{*}{DoS} & Pre-Q          & 0.9992             & 1               & 0.9996    & 0.04\% & 0\%  \\
& MA-QCNN         & 0.9992             & 1               & 0.9996    & 0.04\% & 0\%  \\
%\underline{\textbf{Fuzzy}} &                    &                 &             \\
\multirow{2}{*}{Fuzzy} & Pre-Q          & 0.9966             & 0.9875          & 0.992    & 0.1\% & 1.25\%  \\
& MA-QCNN         & 0.9966             & 0.9878          & 0.9922   & 0.1\% & 1.22\%   \\
\bottomrule
\end{tabular}}
\label{table:preqcomp}\vspace{-10pt}
\end{table}


The model is then packaged as an `xmodel' file which can be executed using a DPU accelerator in the PL with the VART libraries installed on the OS running on the PS. 
For our experiments, we use a petalinux based image for the Ultra-96 V2 board on which the PYNQ and VART libraries were installed to use the standard VART/PYNQ APIs. %  DPU accelerator and to other peripherals on the board. 
Subsequently, the bitstream corresponding to the DPU accelerator is loaded to the PL from the OS (as an overlay). 
For our experiment, we use the B1152 DPU for most of the performance measurements (unless specified) with the DPU using a 150 MHz interface clock and 300 MHz DSP core clock. %\todo[inline]{Are you sure these clocks are correct? I recall that Ultra-96 V2 had issues with current limits and would only work $<$ 195 MHz in cases, or up to 255 MHz with the current limit fixed...: \textcolor{blue}{I should have checked this before. In the block design I have found the clocks that go into the DPU and found the above.}}
%The generated '.h5' file from the above goes through the Vitis-AI toolchain before it can be deployed on the FPGA.
%The model file if first quantised. In this process, the weights, biases and activation of the full precision model are quantised to 8-bits.
%We then test the quantised model again to check to performance degradation.
%If there is major degradation then the post-quantisation finetuning of the quantised model can help address that.
%\todo[inline]{To fix from here: }
%Once fully verified the quantised model is packaged into an '.xmodel' file containing the weights of the quantised model ready for deployment.
%On the FPGA, the sd card is first loaded with a PYNQ image. Vitis-AI libraries are then installed on top of this image to enable interaction with the DPU accelerator.
%Bit file corresponding to the particular DPU configuration is loaded which is specified as an overlay.
%Python APIs in the Vitis-AI framework are then used to write the time-series inputs and read the outputs from the FPGA accelerator.
%The FPGA accelerator (DPU) uses a 300 MHz interface clock and a 600 MHz DSP core clock.
%The tensorflow model is trained on an NVIDIA RTX A6000 GPU. Model quantisation is carried out on an Intel Core i9-10900 CPU (10 cores).

For our evaluation, we compare our model performance in terms of inference accuracy metrics and processing latency with the state of the art IDSs and IPSs described in the literature.
We use Precision, Recall, F1 score, and False Negative Rates (FNR) to compare the inference accuracy of other models where reported and use per-message latency to capture the true latency of the detection approach starting from the arrival of a new CAN message at the interface. 
In case of schemes where inference is performed on a block of CAN messages, this is captured using the block size in the comparison.
We further determine the power consumption of the ECU while executing the IDS and compare it against the execution of the full-precision model on a GPU. 
Note that none of the ML-based IDS approaches in the literature report the actual power consumption of their implementations; however, since most models are significantly more complex than our lightweight model, we assume that our GPU implementation would be a good baseline for comparison.  
%We run the model on different DPU configurations available for experimentation and present a comparison among them.


\subsection{Inference Accuracy}

%Table~\ref{table:preqcomp} shows that the quantisation of the pre-trained full precision model does not lead to performance degradation.
Table~\ref{table:dcnncomp} compares the proposed MA-QCNN with the state of the art approaches discussed in the research literature: GIDS~\cite{seo2018gids}, DCNN~\cite{song2020vehicle}, iForest~\cite{de2021efficient}, MTH-IDS~\cite{yang2021mth}, TCAN-IDS~\cite{cheng2022tcan} \& NovelADS~\cite{agrawal2022novelads}.
In the case of MTH-IDS, the authors only report an average accuracy, precision \& recall of 0.99 across all attacks which is identical to our model on the three metrics.
%\todo[inline]{Not split into individual tests? Else, we Add to the table? Also, trained and tested individually?}
In case of the \textit{DoS attack}, our quantised hardware accelerator performs almost identical to the DCNN, TCAN-IDS, NovelADS, MLIDS across all metrics and has superior performance than GIDS across all metrics.
%\todo[inline]{How can we say it is superior to MLIDS and MTH if we dont know how id did in DoS? Same with fuzzing below? We should average it in a similar fashion and compare?: \textcolor{blue}{Okay. I have made those changes and added MLIDS to the table.}}
In case of the \textit{fuzzing attack}, we observe that DCNN, MLIDS \& NovelADS perform marginally better, with 0.6\%, 0.7\% \& 0.8\% better F1 scores respectively. 
Our model is almost identical to TCAN-IDS in case of fuzzing attacks and offers a marginal improvement over iForest and GIDS by 1.7\% and 0.9\% respectively (F1 scores).
Note that in case of competing techniques, the models are trained afresh for each attack, whereas our model uses an induced learning approach during training and hence, uses the exact weights, biases and activation values for both attacks.%\todo[inline]{Isn't this correct?:\textcolor{blue}{Yes. This is correct.}}

%We are equal to TCAN-IDS and better performing compared to iForest \& GIDS by 1.7\% and 0.9\% respetively.
Table~\ref{table:confmatrix} shows the confusion matrix of MA-QCNN on the two attacks. 
%\todo[inline]{Do we need this? : \textcolor{blue}{Tells the raw numbers of the classifiers. People usually put it.}}
We also plot the ROC curve for the two attacks when using our model on the Ultra-96 V2, which is shown in Figure~\ref{fig:roc}, and further determine the AUC values for our model based on the test datasets.
%Figure~\ref{fig:roc} shows the ROC curves for the two attacks. 
We observe that our model achieves an AUC value $ > $0.99 in both attacks with a slightly lower performance in the fuzzing attack.
We believe that this could be improved by fine-tuning the training and post-quantisation tuning steps.
%\todo[inline]{What is the significance of this? A line specifying this should be here? Or is it implied from the explanation above?}

\begin{table}[t!]
\centering
\caption{Confusion matrix capturing the classification results of the 2-bit MLP.}
    \scalebox{1}{%0.9
        \begin{tabular}{llcrr}
            \toprule
                                  & \multicolumn{4}{c}{\textbf{Predicted Values}} \\
            \cmidrule{2-5}
            \textbf{2-bit Model} & \textbf{Normal}  & \textbf{DoS}  & \textbf{Fuzzing} & \textbf{RPM-Spoof}  \\ 
            \midrule
            \textbf{Normal}   & 103012     &        102                          &   56  &      6                          \\ 
            \textbf{DoS}      &  134   &     23555                             &    4     &      0                  \\ 
            \textbf{Fuzzing}  &  210   &     2                           &      27859    &  18                        \\
            \textbf{RPM-Spoof}  &  2   &       0                         &     0     &   25040                       \\
            \bottomrule
        \end{tabular}}
\label{table:confmatrix-2bit}
\end{table}

% [[103012    102     56      6]
%  [   134  23555      4      0]
%  [   210      2  27859     18]
%  [     2      0      0  25040]]


\begin{table}[t!]
\centering
\caption{Confusion matrix capturing the classification results of the 3-bit MLP.}
    \scalebox{1}{%0.9
        \begin{tabular}{llcrr}
            \toprule
                                  & \multicolumn{4}{c}{\textbf{Predicted Values}} \\
            \cmidrule{2-5}
            \textbf{3-bit Model} & \textbf{Normal}  & \textbf{DoS}  & \textbf{Fuzzing} & \textbf{RPM-Spoof}  \\ 
            \midrule
            \textbf{Normal}   &   103155   &       18                           & 3    &       0                         \\ 
            \textbf{DoS}      &   41  &    23652                              &    0     &     0                   \\ 
            \textbf{Fuzzing}  &  50   &      0                          &     28035     &   4                       \\
            \textbf{RPM-Spoof}  &  0   &          0                      &    0      &            25042              \\
            \bottomrule
        \end{tabular}}
\label{table:confmatrix-3bit}
\end{table}

\begin{table}[t!]
\centering
\caption{Confusion matrix capturing the classification results of the 4-bit MLP.}
    \scalebox{1}{%0.9
        \begin{tabular}{llrr}
            \toprule
                                  & \multicolumn{3}{c}{\textbf{Predicted Values}} \\
            \cmidrule{2-4}
            \textbf{4-bit Model} & \textbf{Normal}  & \textbf{DoS}  & \textbf{Fuzzing}  \\ 
            \midrule
            \textbf{Normal}   &   82129   &         14                         &    6                                 \\ 
            \textbf{DoS}      &   1  &              21532                    &     0                            \\ 
            \textbf{Fuzzing}  &  30  &                0                &        16288                            \\ 
            \bottomrule
        \end{tabular}}
\label{table:confmatrix-4bit}
\end{table}


\begin{table}[t!]
\centering
\caption{Accuracy metric comparison of our quantised FPGA accelerator (MA-QCNN) against the reported literature.}
\scalebox{0.95}{%0.85
\begin{tabular}{@{}llllll@{}}
\toprule
\textbf{Attack}  & \textbf{Model} & \textbf{Precision} & \textbf{Recall} & \textbf{F1}  & \textbf{FNR} \\
\midrule
\multirow{5}{*}{DoS} & GIDS~\cite{seo2018gids}                  & 0.968                & 0.996          & 0.981  &   -   \\ 
& DCNN~\cite{song2020vehicle}                  & 1.0                & 0.9989          & 0.9995  & 0.13\%     \\
& MLIDS~\cite{desta2020mlids}                  & 0.999                & 1          & 0.999  & -     \\
& NovelADS~\cite{agrawal2022novelads}                  & 0.9997               & 0.9991          & 0.9994  & -     \\
& TCAN-IDS~\cite{cheng2022tcan}                  & 1             & 0.9997          & 0.9998  & -     \\
& iForest~\cite{de2021efficient}                  & -                &   -       &  - &  -    \\ 
& \textbf{MA-QCNN (DPU)}                  & 0.9992             & 1               & 0.9996  & 0\%     \\
\midrule
%\underline{\textbf{Fuzzy}} &              &                    &                 &             \\
\multirow{5}{*}{Fuzzing} & GIDS~\cite{seo2018gids}                  & 0.973                & 0.995          & 0.983   & -    \\ 
& DCNN~\cite{song2020vehicle}                 & 0.9995             & 0.9965          & 0.9980  & 0.5\%     \\
& MLIDS~\cite{desta2020mlids}                  & 0.999             & 0.999          & 0.999  & -     \\
& NovelADS~\cite{agrawal2022novelads}                  & 0.9999               & 1         & 1  & -     \\
& TCAN-IDS~\cite{cheng2022tcan}                  & 0.9996             & 0.9989          & 0.9922  & -     \\
& iForest~\cite{de2021efficient}                  & 0.9507                & 0.9993          & 0.9744  &    -  \\
& \textbf{MA-QCNN (DPU)}            & 0.9966             & 0.9878          & 0.9922   & 1.22\%     \\
\bottomrule
\end{tabular}}
\label{table:dcnncomp}\vspace{-10pt}
\end{table}

\begin{figure}[t!]
    \centering
    \includegraphics[scale = 0.45,trim={0cm 1cm 0 1cm},clip]{figures/RoC.pdf}
    \caption{ROC curve of the MA-QCNN on the two attacks.}
    \label{fig:roc}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[scale = 0.45]{figures/chart-5.pdf}
    \caption{Confidence values of the 2-bit model for the four types of messages used in testing.}
    \label{fig:boxplot}
\end{figure}

\subsection{Latency \& Power consumption}
%\todo{Needs fixing...}
To determine the real-time detection performance, we evaluate the processing latency of the inference datapath from the arrival of a new message and compare it against competing approaches in the literature. 
As mentioned before, some approaches perform block-based detection and hence require the block of messages to be available before it is fed as input to the inference engine.
This reduces average inference latency per message leveraging the parallelism on the GPUs.
However, accumulating 64 messages (for example) consumes nearly 8.3\,ms on a 1\,Mbps CAN network with 8-byte messages, which should be factored into their worst-case detection latency when averaging.
The results are shown in table~\ref{table:latcomp}, also capturing the execution platform and the block size in case of block-based inference. 
We can observe the lightweight model on our approach takes 0.43\,ms from the arrival of a message from the CAN interface, which is better than most approaches when measuring the processing time from the arrival of the last message of the block across all platforms.
Finally, our approach does incur additional latency due to message looping through the ECU, and could be reduced further using a CAN interface in the PL feeding the DPU through a FIFO. 
%cut off to reduce the latency further by using the CAN interface data directly or using custom CAN controllers that can stream decoded bits as they are decoded from the bus to the IDS block on the PL.
Also, on a more capable hybrid FPGA, a larger DPU could be configured to have multiple execution units and/or multiple execution threads to reduce latency further at the expense of slightly higher power consumption. 

We also measure the power consumption of the IDS ECU while performing inference, using the PYNQ-PMBus package to monitor the power rails directly. 
All power measurements are averaged over 100 inference runs, each evaluating the test set lasting nearly 10 seconds. 
We observe that the Ultra-96 ECU consumes 2\,W when the CAN messages are been analysed using the DPU block on the PL. 
In comparison, our lightweight floating-point model running on the A6000 consumes 54\,W while performing inference at similar CAN data rates, which is 27$
\times$ higher than the entire IDS ECU on the Ultra-96 device. 
Other IDS implementations in the literature do not report power measurements; however, our lightweight model on the GPU should be a good baseline and more complex models discussed in the literature should consume higher power during inference on GPUs.
Thus, our IDS ECU on a hybrid FPGA like an Ultra-96 device offers an ideal mix of detection accuracy, latency, power consumption, while offering software-driven control of IDS and seamless GPU-like deployment with minimal change to the ECU application, making it an ideal choice for in-vehicle deployment.

%% Our approach uses a moving window approach using a FIFO-style input buffer, and is hence more reactive to every new message.
%% We compare the per-message processing latency of the proposed implementation with the following works: %% ~\cite{seo2018gids,desta2020mlids,song2020vehicle,agrawal2022novelads,cheng2022tcan,yang2021mth} as shown in table~\ref{table:latcomp}.
%% In~\cite{desta2020mlids}, the authors report a per message latency of 275ms when the model is executed on a  Nvidia GTX Titan X (GM200) GPU.
%% In~\cite{cheng2022tcan},~\cite{song2020vehicle},~\cite{seo2018gids}\&~\cite{agrawal2022novelads} the authors operate on a block of CAN message and report a %% latency of 3.4ms, 5ms, 5.89ms \& 128.72ms when executed on the Nvidia Jetson AGX Xavier, Tesla K80, GeForce GTX 1080 \& Jetson Nano GPUs respectively. 
%% This leads to an average processing latency of 0.05ms, 0.17ms, 0.09ms \& 1.28ms respectively at the expense of a higher waiting time for the arrival of the %% block of messages.
%% The number of cuda cores available on the above GPUs is also shown table~\ref{table:latcomp}. 
%% %\todo[inline]{Are these the values after hyphen? Better to use the GPU name, so they can go and look up if needed? : \textcolor{blue}{Okay. I thought it %% would like nice in the table. I have replaced them with their names.}}
%% In~\cite{yang2021mth}, the authors report a per-message latency of 0.574ms when their lightweight multi-model stacked IDS is executed on a Raspberry Pi 3 %% machine.
%% Thus, our integrated IDS (Zynq:70k-LUTs)-ECU approach offers the lowest per-message latency in comparison with the other state of the art IDSs.
%% 
%% We also quantify the power consumption of our system by monitoring the power rails on the device through the PYNQ-PMBus package. 
%% %This package allows us to record power on different voltage lines of interest on the board. 
%% %All power rails of interest were monitored during the test to determine the
%% We observe our idle/active power consumption using this, monitoring all the power rails of interest. 
%% For the B1152 DPU, we observe the active power consumption to be 2\,W with the PS running at high-power active mode. 
%% This is significantly lower than the power estimates from GPU acceleration of our light-weight full precision model which consumed 54\,W on an Nvidia A6000 %% GPU.
%% We estimate that this integrated approach is significantly more power efficient than state of the art IDS on GPU or standalone CPUs. 
%% %We find the active power consumed to be 2.23W making it quite suitable for the edge. 
%The IDS meets the deployment needs of in-vehicle networks both in terms of latency and power consumption.
%For a lower power consumption the arm cores can also be set to operate on a low power mode bringing the consumption down to 1.77W. 
%% NOTE: unless you set it explicitly to low-power mode, this rail will not give you the right value.. as you see, the PL only takes about  0.3\,W and low-power mode on arm should be a few 100 mW. - see here: https://docs.xilinx.com/v/u/en-US/wp482-zu-pwr-perf

\begin{table}[t!]
\centering
\caption{Per-message latency comparison against state of the art IDSs (GPU/Raspberry Pi) reported in literature.}
\scalebox{0.9}{%0.9
\begin{tabular}{@{}lrll@{}}
\toprule
\textbf{Models}     & \textbf{Latency} & \textbf{Frames} & \textbf{Platform} \\ \cmidrule{1-4}
MLIDS & 275\,ms & per CAN frame & GTX Titan X \\%GPU-3072\\
NovelADS & 128.7\,ms & 100 CAN frames & Jetson Nano \\%GPU-128\\
GIDS & 5.89\,ms & 64 CAN frames &  GTX 1080  \\%GPU-2560 \\ 
DCNN &  5\,ms & 29 CAN frames & Tesla K80 \\%GPU-2496      \\
TCAN-IDS & 3.4\,ms & 64 CAN frames & Jetson AGX \\%GPU-512 \\
MTH-IDS~\cite{yang2021mth} &  0.574\,ms & per CAN frame & Raspberry Pi 3     \\
\textbf{MA-QCNN (DPU)} & 0.43\,ms & per CAN frame & Zynq FPGA    \\ 
\bottomrule
\end{tabular}}
\label{table:latcomp}\vspace{-10pt}
\end{table}


% \begin{table}[t!]
% \centering
% \caption{Resource utilization breakdown for PL Accelerator of our proposed CAN IDS (XCZU3EG).}
% \scalebox{1}{
% \begin{tabular}{lrrrr}
% \toprule
% \textbf{Node} & \textbf{LUT} & \textbf{FF} & \textbf{BRAM} & \textbf{DSP} \\
% \midrule
% DPU           & 32934        &  57536           & 127.5            & 312  \\
% \midrule
% Overall & 70560  & 141120  & 216  & 360 \\
% (\% usage) & (46.6\%) & (40.7\%) & (59\%) & (86.6\%) \\
% \bottomrule
% \end{tabular}}
% %\vspace*{0.1cm}
% \label{table:resourceutilization}
% %\vspace{-10pt}
% \end{table}

%% \subsection{Different DPU configurations}
%% \todo[inline]{Do we need all cases here? can we just do the B512,B1152 and B2304? and say that B1152 is the best option? - Also, we do not go into threading right? And two-cores per DPU? %% :\textcolor{blue}{ Yes we can do 3 configs only. No multithreading does not imptove the latency much. It is single core per DPU.}}
%% On the Ultra96-V2, due to resource constraints; 6 out of the total 8 DPUs available for experimentation can be executed.
%% Table~\ref{table:dpucomparison} shows the latency, \% resource utilisation and power consumption of the MA-QCNN when executed on the DPUs.
%% %B2304 DPU is built with low DSP usage so that it can fit on the board.
%% We observe a 10\% reduction in latency as we go from the lowest (B512) to the highest performing DPU (B2304).
%% This comes at a cost of 25.2\% rise in power consumption.


% \begin{table}[t!]
% \centering
% \caption{Performance scaling of the MA-QCNN model using different DPU configurations: impact on per message latency (ms), resource (\%), \& power consumption (W).}
% \scalebox{1}{
% \begin{tabular}{lcccccccr}
% \toprule
% \multirow{2}{*}{\textbf{DPU}} & \multirow{2}{*}{\textbf{Latency}} & \multicolumn{4}{c}{\textbf{\% Resource Utilisation}} & \multicolumn{2}{c}{\textbf{Power (W)}} \\ \cmidrule{3-8}
%  & (ms) & LUT & FF & DSP & BRAM & Idle & Active \\ \midrule
% B512           & 0.48                 & 35   & 25.3  & 30.5 & 34 & 1.53  &1.78  \\
% B800           &  0.44               & 39.2  &30.1 & 43.6 &42.3  &  1.55&1.82   \\
% B1024           & 0.48               & 43.9 &35 &60.5 &48.8 & 1.67&2.01    \\
% B1152           &  0.43               & 43.8 & 34.5&58.8 &56.9 & 1.69&2   \\
% B1600           & 0.44          & 49.4  & 42.8 & 86.6 & 59 & 1.79 & 2.15  \\
% B2304           &  0.43               & 59.6 &53.6 &90.5 &77.3 &1.9 &2.23   \\
% \bottomrule
% \end{tabular}}
% \label{table:dpucomparison}
% \end{table}

==> relatedworks.tex <==
\section{Related Works} \label{rel_work}



==> tables/CNN.tex <==
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.5}
\begingroup
\begin{table}[h]\scriptsize
\begin{tabular}{lcccc}
\hline
                                      & \textbf{\begin{tabular}[c]{@{}c@{}}Throughput\\ GOps/Sec\end{tabular}}           & \textbf{\begin{tabular}[c]{@{}c@{}}Performance \\ Density\\ GOps/KLUTs\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Precision\\ Fixed-Point\end{tabular}}           & \textbf{\begin{tabular}[c]{@{}c@{}}Frequency\\ MHz\end{tabular}}               \\ \hline
\multicolumn{1}{l|}{\textbf{AlexNet}} & 1200                                                                             & 5.38                                                                                 & 16 bits=8,8                                                                        & 166                                                                            \\ \cline{1-1}
\multicolumn{1}{l|}{\textbf{VGG-16}}  & 1025                                                                             & 4.60                                                                                 & 16 bits=8,8                                                                        & 166                                                                            \\ \hline
                                      & \textbf{\begin{tabular}[c]{@{}c@{}}Execution\\ Kilo Cycles \\ (EC)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Memory\\ Kilo Cycles \\ (MC)\end{tabular}}        & \textbf{\begin{tabular}[c]{@{}c@{}}Theoretical\\ Kilo Cycles \\ (TC)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Pipeline \\ Rate\\ (EC+MC)/TC\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\textbf{AlexNet}} & 1096                                                                             & 112                                                                                  & 856                                                                                & 1.45                                                                           \\ \cline{1-1}
\multicolumn{1}{l|}{\textbf{VGG-16}}  & 7046                                                                             & 431                                                                                  & 5149                                                                               & 1.44                                                                           \\ \hline
\end{tabular}
\caption{The table lists the Execution Cycles (EC), Memory Cycles (MC) and Theoretical Cycles (TC) required by our overlay to process various networks. The pipeline rate (PR) to process each network is also reported. }
\label{tab:scale_cnn}
\end{table}
\endgroup

==> tables/resr_utilisation.tex <==
\renewcommand{\arraystretch}{1.5}
\begin{table}[]
\centering
\begin{tabular}{cccc}
\hline
\textbf{Method}                        & \textbf{Adders}   & \textbf{Freq.(MHz)} & \textbf{Slices} \\ \hline
\multicolumn{1}{c|}{\textbf{FCBT}~\cite{zhuo2007high}}     & 2                 & 170                 & 2859            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{DSA}~\cite{zhuo2007high}}      & 2                 & 142                 & 2215            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{SSA}~\cite{zhuo2007high}}      & 1                 & 165                 & 1804            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{DB}~\cite{tai2011accelerating}}       & 1                 & 188                 & 1749            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{MFPA}~\cite{huang2012modular}}     & 5                 & 207                 & 4491            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{AeMFPA}~\cite{huang2012modular}}   & 2                 & 204                 & 3130            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{Ae$^2$MFPA}~\cite{huang2012modular}}   & 2                 & 144                 & 3737            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{SBM}~\cite{tang2019resource}}      & 1                 & 278                 & 1670            \\ \cline{1-1}
\multicolumn{1}{c|}{\textbf{TreeNet}} & \textbf{36 (FxPt)} & \textbf{200}        & \textbf{5854}   \\ \hline
\end{tabular}
\caption{Table compares the slice consumption of TreeNet along the operating frequency with other works.}
\label{tab:adder-table}
\end{table}

==> tables/util_improv.tex <==
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.3}
\begin{table}[]\scriptsize
\centering
\begin{tabular}{l|cccccccccccc|}
\cline{2-13}
                                   & \multicolumn{3}{c|}{\textbf{3 x 3}} & \multicolumn{3}{c|}{\textbf{5 x 5}} & \multicolumn{3}{c|}{\textbf{7 x 7}} & \multicolumn{3}{c|}{\textbf{9 x 9}} \\ \cline{2-13} 
\multicolumn{1}{c|}{}              & LUT        & FF         & RAM       & LUT        & FF         & RAM       & LUT        & FF         & RAM       & LUT        & FF         & RAM       \\ \hline
\multicolumn{1}{|l|}{\textbf{1}}   & 2.5x       & 2.1x       & 1.3x      & 2.2x       & 2.2x       & 1.3x      & 2.4x       & 2.8x       & 1.6x      & 2.2x       & 2.6x       & 1.4x      \\
\multicolumn{1}{|l|}{\textbf{2}}   & 2.3x       & 1.9x       & 1.2x      & 1.9x       & 1.9x       & 1.2x      & 2.2x       & 2.4x       & 1.5x      & 2.0x       & 2.1x       & 1.3x      \\
\multicolumn{1}{|l|}{\textbf{4}}   & 2.0x       & 1.9x       & 0.9x      & 1.8x       & 1.9x       & 0.9x      & 2.1x       & 2.4x       & 1.2x      & 1.8x       & 1.8x       & 1.1x      \\
\multicolumn{1}{|l|}{\textbf{8}}   & 1.9x       & 2.0x       & 1.1x      & 1.9x       & 2.1x       & 1.2x      & 2.3x       & 2.3x       & 1.6x      & 2.2x       & 1.9x       & 1.5x      \\
\multicolumn{1}{|l|}{\textbf{16}}  & 2.0x       & 2.2x       & 1.2x      & 1.9x       & 2.3x       & 1.5x      & 2.4x       & 2.5x       & 2.0x      & 2.5x       & 2.3x       & 2.1x      \\
\multicolumn{1}{|l|}{\textbf{32}}  & 2.0x       & 2.3x       & 1.1x      & 1.8x       & 2.5x       & 1.5x      & 2.3x       & 2.7x       & 1.9x      & 1.7x       & 1.7x       & 2.2x      \\
\multicolumn{1}{|l|}{\textbf{64}}  & 2.2x       & 2.5x       & 1.1x      & 1.9x       & 2.7x       & 1.5x      & 2.2x       & 2.5x       & 1.9x      & 2.0x       & 2.0x       & 2.2x      \\
\multicolumn{1}{|l|}{\textbf{128}} & 2.2x       & 2.6x       & 1.1x      & 2.0x       & 2.7x       & 1.5x      & 2.2x       & 2.5x       & 1.9x      & 2.1x       & 2.2x       & 2.3x      \\
\multicolumn{1}{|l|}{\textbf{256}} & 2.3x       & 2.7x       & 1.1x      & 2.1x       & 2.7x       & 1.5x      & 2.3x       & 2.5x       & 2.0x      & 2.1x       & 2.2x       & 2.4x      \\
\multicolumn{1}{|l|}{\textbf{512}} & 2.7x       & 2.9x       & 1.1x      & 2.4x       & 2.1x       & 1.5x      & 2.6x       & 3.0x       & 2.0x      & 3.4x       & 3.3x       & 2.4x      \\ \hline
\end{tabular}
\caption{Absolute resource numbers for the presented approach.}
\end{table}

==> tables/utilization.tex <==
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.3}
\begin{table*}[]\scriptsize
\centering
\begin{tabular}{cccccccccccccl}
\multicolumn{13}{c}{\textbf{(a) Our Work}}                                                                                                                                                                                                                                                                                                           &  \\ \cline{1-13}
\multicolumn{1}{|c|}{\textbf{Replications}} & \multicolumn{3}{c|}{\textbf{3 x 3}}                                      & \multicolumn{3}{c|}{\textbf{5 x 5}}                                      & \multicolumn{3}{c|}{\textbf{7 x 7}}                                    & \multicolumn{3}{c|}{\textbf{9 x 9}}                                     &  \\ \cline{1-13}
\multicolumn{1}{|c|}{}                      & LUT                  & FF                   & \multicolumn{1}{c|}{RAM}   & LUT                  & FF                   & \multicolumn{1}{c|}{RAM}   & LUT                  & FF                   & \multicolumn{1}{c|}{RAM} & LUT                  & FF                   & \multicolumn{1}{c|}{RAM}  &  \\ \cline{2-13}
\multicolumn{1}{|c|}{1}                     & 167                  & 299                  & \multicolumn{1}{c|}{3}     & 270                  & 410                  & \multicolumn{1}{c|}{4.5}   & 327                  & 446                  & \multicolumn{1}{c|}{5}   & 459                  & 637                  & \multicolumn{1}{c|}{7}    &  \\
\multicolumn{1}{|c|}{2}                     & 195                  & 371                  & \multicolumn{1}{c|}{4}     & 324                  & 522                  & \multicolumn{1}{c|}{5.5}   & 375                  & 592                  & \multicolumn{1}{c|}{6}   & 551                  & 887                  & \multicolumn{1}{c|}{8}    &  \\
\multicolumn{1}{|c|}{4}                     & 268                  & 514                  & \multicolumn{1}{c|}{5.5}   & 417                  & 697                  & \multicolumn{1}{c|}{7.5}   & 454                  & 785                  & \multicolumn{1}{c|}{7}   & 676                  & 1272                 & \multicolumn{1}{c|}{10}   &  \\
\multicolumn{1}{|c|}{8}                     & 414                  & 798                  & \multicolumn{1}{c|}{9}     & 610                  & 1044                 & \multicolumn{1}{c|}{11}    & 653                  & 1204                 & \multicolumn{1}{c|}{11}  & 843                  & 1771                 & \multicolumn{1}{c|}{14}   &  \\
\multicolumn{1}{|c|}{16}                    & 681                  & 1363                 & \multicolumn{1}{c|}{16}    & 981                  & 1737                 & \multicolumn{1}{c|}{18}    & 1017                 & 2023                 & \multicolumn{1}{c|}{18}  & 1209                 & 2717                 & \multicolumn{1}{c|}{21}   &  \\
\multicolumn{1}{|c|}{32}                    & 1220                 & 2489                 & \multicolumn{1}{c|}{30.5}  & 1708                 & 3127                 & \multicolumn{1}{c|}{32}    & 1734                 & 3659                 & \multicolumn{1}{c|}{32}  & 2740                 & 6851                 & \multicolumn{1}{c|}{35}   &  \\
\multicolumn{1}{|c|}{64}                    & 2133                 & 4757                 & \multicolumn{1}{c|}{59}    & 3154                 & 5897                 & \multicolumn{1}{c|}{60.5}  & 3425                 & 8064                 & \multicolumn{1}{c|}{61}  & 4485                 & 11681                & \multicolumn{1}{c|}{64}   &  \\
\multicolumn{1}{|c|}{128}                   & 4392                 & 9344                 & \multicolumn{1}{c|}{116}   & 6226                 & 12100                & \multicolumn{1}{c|}{117.5} & 6839                 & 16037                & \multicolumn{1}{c|}{118} & 8458                 & 22210                & \multicolumn{1}{c|}{120}  &  \\
\multicolumn{1}{|c|}{256}                   & 8964                 & 18823                & \multicolumn{1}{c|}{229.5} & 12407                & 24716                & \multicolumn{1}{c|}{231.5} & 13722                & 32998                & \multicolumn{1}{c|}{231} & 17200                & 45615                & \multicolumn{1}{c|}{234}  &  \\
\multicolumn{1}{|c|}{512}                   & 15526                & 36308                & \multicolumn{1}{c|}{457}   & 21916                & 46210                & \multicolumn{1}{c|}{459}   & 24938                & 65388                & \multicolumn{1}{c|}{459} & 21816                & 60139                & \multicolumn{1}{c|}{462}  &  \\ \cline{1-13}
\multicolumn{1}{l}{}                        & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}      &  \\
\multicolumn{13}{c}{\textbf{(b) FPGA 2018 }}                                                                                                                                                                                                                                                                                                 &  \\ \cline{1-13}
\multicolumn{1}{|c|}{\textbf{Replications}} & \multicolumn{3}{c|}{\textbf{3 x 3}}                                      & \multicolumn{3}{c|}{\textbf{5 x 5}}                                      & \multicolumn{3}{c|}{\textbf{7 x 7}}                                    & \multicolumn{3}{c|}{\textbf{9 x 9}}                                     &  \\ \cline{1-13}
\multicolumn{1}{|c|}{}                      & LUT                  & FF                   & \multicolumn{1}{c|}{RAM}   & LUTs                 & FF                   & \multicolumn{1}{c|}{RAM}   & LUT                  & FF                   & \multicolumn{1}{c|}{RAM} & LUT                  & FF                   & \multicolumn{1}{c|}{RAM}  &  \\ \cline{2-13}
\multicolumn{1}{|c|}{1}                     & 425                  & 631                  & \multicolumn{1}{c|}{4}     & 602                  & 917                  & \multicolumn{1}{c|}{6}     & 805                  & 1278                 & \multicolumn{1}{c|}{8}   & 1040                 & 1695                 & \multicolumn{1}{c|}{10}   &  \\
\multicolumn{1}{|c|}{2}                     & 461                  & 704                  & \multicolumn{1}{c|}{5}     & 638                  & 1032                 & \multicolumn{1}{c|}{7}     & 859                  & 1428                 & \multicolumn{1}{c|}{9}   & 1107                 & 1891                 & \multicolumn{1}{c|}{11}   &  \\
\multicolumn{1}{|c|}{4}                     & 560                  & 990                  & \multicolumn{1}{c|}{5}     & 763                  & 1366                 & \multicolumn{1}{c|}{7}     & 996                  & 1952                 & \multicolumn{1}{c|}{9}   & 1264                 & 2377                 & \multicolumn{1}{c|}{11}   &  \\
\multicolumn{1}{|c|}{8}                     & 823                  & 1632                 & \multicolumn{1}{c|}{10}    & 1158                 & 2252                 & \multicolumn{1}{c|}{14}    & 1528                 & 2856                 & \multicolumn{1}{c|}{18}  & 1911                 & 3484                 & \multicolumn{1}{c|}{22}   &  \\
\multicolumn{1}{|c|}{16}                    & 1379                 & 3017                 & \multicolumn{1}{c|}{20}    & 1925                 & 4121                 & \multicolumn{1}{c|}{28}    & 2489                 & 5231                 & \multicolumn{1}{c|}{36}  & 3059                 & 6354                 & \multicolumn{1}{c|}{44}   &  \\
\multicolumn{1}{|c|}{32}                    & 2444                 & 5919                 & \multicolumn{1}{c|}{35}    & 3216                 & 8070                 & \multicolumn{1}{c|}{49}    & 3997                 & 10176                & \multicolumn{1}{c|}{63}  & 4742                 & 12284                & \multicolumn{1}{c|}{77}   &  \\
\multicolumn{1}{|c|}{64}                    & 4826                 & 11967                & \multicolumn{1}{c|}{65}    & 6265                 & 16119                & \multicolumn{1}{c|}{91}    & 7711                 & 20290                & \multicolumn{1}{c|}{117} & 9218                 & 24465                & \multicolumn{1}{c|}{143}  &  \\
\multicolumn{1}{|c|}{128}                   & 10001                & 24661                & \multicolumn{1}{c|}{130}   & 12747                & 32879                & \multicolumn{1}{c|}{182}   & 15494                & 41194                & \multicolumn{1}{c|}{234} & 18306                & 49486                & \multicolumn{1}{c|}{286}  &  \\
\multicolumn{1}{|c|}{256}                   & 20704                & 51117                & \multicolumn{1}{c|}{260}   & 26262                & 67636                & \multicolumn{1}{c|}{364}   & 31603                & 83955                & \multicolumn{1}{c|}{468} & 37062                & 100310               & \multicolumn{1}{c|}{572}  &  \\
\multicolumn{1}{|c|}{512}                   & 43360                & 106385               & \multicolumn{1}{c|}{515}   & 54097                & 100000               & \multicolumn{1}{c|}{721}   & 64928                & 200000               & \multicolumn{1}{c|}{927} & 75862                & 204114               & \multicolumn{1}{c|}{1133} &  \\ \cline{1-13}
\end{tabular}
\caption{Absolute resource numbers for the presented approach.}
\end{table*}
